Unravelling New Physics Signals at the HL-LHC with Low-Energy Constraints

Recent studies suggest that global fits of Parton Distribution Functions (PDFs) might inadvertently 'fit away' signs of new physics in the high-energy tails of the distributions measured at the high luminosity programme of the LHC (HL-LHC). This could lead to spurious effects that might conceal key BSM signatures and hinder the success of indirect searches for new physics. In this letter, we demonstrate that future deep-inelastic scattering (DIS) measurements at the Electron-Ion Collider (EIC), and at CERN via FASER$\nu$ and SND@LHC at LHC Run III, and the future neutrino experiments to be hosted at the proposed Forward Physics Facility (FPF) at the HL-LHC, provide complementary constraints on large-$x$ sea quarks. These constraints are crucial to mitigate the risk of missing key BSM signals, by enabling precise constraints on large-$x$ PDFs through a 'BSM-safe' integration of both high- and low-energy data, which is essential for a robust interpretation of the high-energy measurements.

==> tables/EIC_data.tex <==
\begin{table}[ht!]
\centering
\footnotesize
\setlength{\tabcolsep}{16pt} % Increase the space between columns. Adjust the value as needed.
\renewcommand{\arraystretch}{1.5} % Increase the space between lines.
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Observable} $\quad$ & $N_{dat}$ & $\sqrt{s}$ [GeV] & $\mathcal{L}$ [fb$^-1$] \\

\hline
\textbf{Charged Current} & & & \\
$\tilde{\sigma}(e^- + p \rightarrow \nu + X)$ & 89 (89) & 140.7 & 100 \\
$\tilde{\sigma}(e^+ +p \rightarrow \bar{\nu} + X)$ & 89 (89) & 140.7 & 10 \\


 \hline
 \textbf{Neutral Current (proton)} & & &\\
$\tilde{\sigma}(e^- + p \rightarrow e^- + X)$ & 181 (131) & 140.7 & 100 \\
& 181 (131) & 63.2 & 100 \\
& 126 (91) & 44.7 & 100 \\
& 87 (76) & 28.6 & 100 \\
$\tilde{\sigma}(e^+ + p \rightarrow e^+ + X)$ & 181 (131) & 140.7 & 10 \\
& 181 (131) & 63.2 & 10 \\
& 126 (91) & 44.7 & 10 \\
& 87 (76) & 28.6 & 10 \\

 \hline
 \textbf{Neutral Current (deuteron)} & & &\\
$\tilde{\sigma}(e^- + d \rightarrow e^- + X)$ & 116 (116) & 89.0 & 10 \\
& 107 (107) & 66.3 & 10 \\
& 76 (76) & 28.6 & 10 \\
$\tilde{\sigma}(e^+ + d \rightarrow e^+ + X)$& 116 (116) & 89.0 & 10 \\
& 107 (107) & 66.3 & 10 \\
& 76 (76) & 28.6 & 10 \\


 \hline

\end{tabular}
\caption{Presentation of the EIC projection data. We use the projected cross-section of NC and CC processes and for proton and deuteron targets. $N_{dat}$ is the number of data points in the optimistic (pessimistic) scenario.}
\label{tab:EIC_data}
\end{table}


==> tables/FPF_data.tex <==
\begin{table}[ht!]
    \centering
    \footnotesize
    \setlength{\tabcolsep}{10pt} % Increase the space between columns. Adjust the value as needed.
    \renewcommand{\arraystretch}{1.5} % Increase the space between lines.
    \begin{tabular}{|c|c|}
        \hline
        Observable $\quad$ & $N_{dat}$\\
        
        \hline
        \textbf{FASER$\nu$} & \\
        $\tilde{\sigma}(\nu + N \rightarrow l^- + X)$ & 22  \\
        $\tilde{\sigma}(\bar{\nu} + N \rightarrow l^+ + X)$ & 16  \\
        
        \hline
        \textbf{FASER$\nu$2} & \\
        $\tilde{\sigma}(\nu + N \rightarrow l^- + X)$ & 44  \\
        $\tilde{\sigma}(\bar{\nu} + N \rightarrow l^+ + X)$ & 39  \\
        $\tilde{\sigma}(\nu + N \rightarrow l^- + c/\bar{c} + X)$ & 38  \\
        $\tilde{\sigma}(\bar{\nu} + N \rightarrow l^+ + c/\bar{c} + X)$ & 30  \\

        \hline
        \textbf{AdvSND} & \\
        $\tilde{\sigma}(\nu + N \rightarrow l^- + X)$ & 33  \\
        $\tilde{\sigma}(\bar{\nu} + N \rightarrow l^+ + X)$ & 29  \\
        $\tilde{\sigma}(\nu + N \rightarrow l^- + c/\bar{c} + X)$ & 17  \\
        
        
        \hline
    
    \end{tabular}
\caption{Presentation of the FPF projection data used in this study. The name corresponds to the dataset implementation in the fit. Each of them is associated to a DIS process, where N is a free nucleon assumed to be an isoscalar.}
\label{tab:FPF_data}
\end{table}
    

==> tables/FTDY_data.tex <==
\begin{table}[ht!]
\centering
\footnotesize
\setlength{\tabcolsep}{16pt} % Increase the space between columns. Adjust the value as needed.
\renewcommand{\arraystretch}{1.5} % Increase the space between lines.
\begin{tabular}{|c|c|c|}
\hline
\textbf{Observable} $\quad$ & $N_{dat}$ & $\sqrt{s}$ [GeV] \\

\hline
\textbf{Charged Current} & & \\
$d\sigma_{Z/\gamma^{*}}/dM_{ll}$ (deuteron target)& 15 & 800 \\
$d\sigma_{Z/\gamma^{*}}/dM_{ll}$ (proton target) & 184 & 800 \\
$d\sigma_{Z/\gamma^{*}}/dM_{ll}$ & 119 & 38.8 \\
$d\sigma_{Z/\gamma^{*}}/dM_{ll}$ (deuteron target) & 6 & 120 \\



 \hline

\end{tabular}
\caption{Presentation of the FTDY data.}
\label{tab:FTDY_data}
\end{table}


==> tables/HLLHC_DY_data.tex <==
\begin{table}[ht!]
\centering
\footnotesize
\setlength{\tabcolsep}{10pt} % Increase the space between columns. Adjust the value as needed.
\renewcommand{\arraystretch}{1.5} % Increase the space between lines.
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Observable} $\quad$ & $N_{dat}$ & $\sqrt{s}$ [TeV] & $\mathcal{L}$ [ab$^-1$] \\

\hline
\textbf{Charged Current} & & & \\
$d\sigma_{W^\pm \rightarrow e \nu}/dM_{T}$ & 16 & 14 & 6 \\
$d\sigma_{W^\pm \rightarrow \mu \nu}/dM_{T}$ & 16 & 14 & 6 \\

\hline
\textbf{Neutral Current} & & & \\
$d\sigma_{Z/\gamma^{*} \rightarrow e^+ e^-}/dM_{ll}$ & 12 & 14 & 6 \\
$d\sigma_{Z/\gamma^{*} \rightarrow \mu^+ \mu^-}/dM_{ll}$ & 12 & 14 & 6 \\




 \hline

\end{tabular}
\caption{Presentation of the HLLHC data.}
\label{tab:HLHC_data}
\end{table}


==> tables/HMDY_data.tex <==
\begin{table}[ht!]
\centering
\footnotesize
\setlength{\tabcolsep}{10pt} % Increase the space between columns. Adjust the value as needed.
\renewcommand{\arraystretch}{1.5} % Increase the space between lines.
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Observable} $\quad$ & $N_{dat}$ & $\sqrt{s}$ [TeV] & $\mathcal{L}$ [fb$^-1$] \\

\hline
\textbf{ATLAS} & & & \\
% $\tilde{\sigma}(e^- + p \rightarrow \nu + X)$ & 89 (89) & 140.7 & 100 \\
$d\sigma_{Z/\gamma^{*}}/dM_{ll}$ & 13 & 7 & 49 \\
$d^2\sigma/dm_{\ell\ell}d|y_{\ell\ell}|$ & 48 & 8 & 20.3 \\


 \hline
 \textbf{CMS} & & &\\
 $d\sigma_{Z/\gamma^{*} \rightarrow \mu^+ \mu^-}/dy$ & 132 & 7 & 4.5 \\
 $d\sigma_{Z/\gamma^{*} \rightarrow e^+ e^-}/dy$ & 132 & 7 & 4.8 \\
 $d\sigma_{Z/\gamma^{*}}/dM_{ll}$ & 43 & 13 & 5.1 \\




 \hline

\end{tabular}
\caption{Presentation of the HMDY data.  $N_{dat}$ is the number of data points. We specify the center-of-mass energy $\sqrt{s}$ and the integrated luminosity $\mathcal{L}$ for each of them.}
\label{tab:HMDY_data}
\end{table}


==> tables/mwp_values.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[h]
  \centering
  \small
  \setlength{\tabcolsep}{4pt} % Increase the space between columns. Adjust the value as needed.
  \renewcommand{\arraystretch}{1.2} % Increase the space between lines.
   \begin{tabular}{|c|c|c|c|}
      \hline
Projection data added	   &  $M^{\rm cont}_{W'}$ (TeV) & $\chi^2_{\rm cont}$ & $\chi^2_{\rm bas}$   \\
\hline
%
HL-LHC             &  13.8  &  1.0  &  1.1   \\
HL-LHC + EIC       &  15.9  &  1.6  &  1.0  \\
HL-LHC + FPF       &  17.4  &  1.4  &  1.1  \\
HL-LHC + EIC + FPF &  19.5  &  1.4  &  1.1  \\
\hline
  \end{tabular}
   \caption{\small First column lists the masses $M^{\rm cont}_{W'}$ corresponding to the maximal contamination for each dataset. Second columns shows the associated average $\chi^2$ values. Third column displays the $\chi^2$ of the baseline fits for comparison.}
  \label{tab:mwp}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> tables/mwp_values_simple.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{tabular}{|c|c|c|c|}
      \hline
Projection data added	   &  $M^{\rm cont}_{W'}$ (TeV) & $\chi^2_{\rm cont}$ & $\chi^2_{\rm bas}$   \\
\hline
%
HL-LHC             &  13.8  &  1.0  &  1.1   \\
HL-LHC + EIC       &  15.9  &  1.6  &  1.0  \\
HL-LHC + FPF       &  17.4  &  1.4  &  1.1  \\
HL-LHC + EIC + FPF &  19.5  &  1.4  &  1.1  \\
\hline
\end{tabular}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

